ATLAS: A Model of Short-term European Electricity Market Processes under Uncertainty -- Balancing Modules

The ATLAS model simulates the various stages of the electricity market chain in Europe, including the formulation of offers by different market actors, the coupling of European markets, strategic optimization of production portfolios and, finally, real-time system balancing processes. ATLAS was designed to simulate the various electricity markets and processes that occur from the day ahead timeframe to real-time with a high level of detail. Its main aim is to capture impacts from imperfect actor coordination, evolving forecast errors and a high-level of technical constraints -- both regarding different production units and the different market constraints. This working paper describes the simulated balancing processes in detail and is the second part of the ATLAS documentation.

==> Notes.tex <==
\chapter{Notes}

\begin{itemize}
	\item Change to book format (add chapters)
	\item Get rid of deltas (on delta qs in Market Clearing)
	\item Look for better method of indexation for order coupling
	\item Change Spot to Day Ahead
	\item Make Aggregation box orange
	\item Reorganize: Put Portfolio Optimization right after Market Clearing with the full description of the problem. Then call from there for DAO, etc. 
\end{itemize}

